Deep Reinforced Attention Regression for Partial Sketch Based Image Retrieval

Fine-Grained Sketch-Based Image Retrieval (FG-SBIR) aims at finding a specific image from a large gallery given a query sketch. Despite the widespread applicability of FG-SBIR in many critical domains (e.g., crime activity tracking), existing approaches still suffer from a low accuracy while being sensitive to external noises such as unnecessary strokes in the sketch. The retrieval performance will further deteriorate under a more practical on-the-fly setting, where only a partially complete sketch with only a few (noisy) strokes are available to retrieve corresponding images. We propose a novel framework that leverages a uniquely designed deep reinforcement learning model that performs a dual-level exploration to deal with partial sketch training and attention region selection. By enforcing the model's attention on the important regions of the original sketches, it remains robust to unnecessary stroke noises and improve the retrieval accuracy by a large margin. To sufficiently explore partial sketches and locate the important regions to attend, the model performs bootstrapped policy gradient for global exploration while adjusting a standard deviation term that governs a locator network for local exploration. The training process is guided by a hybrid loss that integrates a reinforcement loss and a supervised loss. A dynamic ranking reward is developed to fit the on-the-fly image retrieval process using partial sketches. The extensive experimentation performed on three public datasets shows that our proposed approach achieves the state-of-the-art performance on partial sketch based image retrieval.

==> back.tex <==
By using policy gradient training and supervised training with hybrid reinforcement loss (also called locator loss) and mse loss (also called action loss), we can get the final sketch representation, searching it in the candidate image gallery, high-performance SBIR can be achieved.

 People can also think FG-SBIR as a zero shot problem\cite{b7}. In training process, it's an N-way 1-shot problem, where N is number of candidate images in the image training set, 1-shot indicates that there is only one ground-truth image corresponding to the query sketch. And at test time, we use new sketch-image pairs which never appear in the training process. \hitesh{The connection between paragraphs Compared to ... image pairs, and People can ..... is not obvious.}
 
 
 
 \subsubsection{Experiment Setting}
\begin{itemize}
    \item Triplet Network:
    The input to the triplet network is a triplet group of one sketch, one positive image and one negative image, all with size 299*299*3. The backbone network of the triplet network is resnet-18 or inceptionV3 . We add an embedding layer with 64 neurons on the top of the feature extractor and we normalize the outputs (l2-norm). On the other side, these features are also passed to attention layers to generate a soft attention mask, then we multiply both sides element-wisely to get the final embedding vector. A triplet loss that can be used for gradient descent. 
    \item Retina and Location encoding:
    The retina encoding $\rho(x;l)$ extracts k square patches centered at
    location l, with the first patch being $g_w \times g_w$ pixels in size, and each successive patch having twice the width of the previous. The k patches are then all resized to $g_w \times g_w$ and concatenated. Glimpse locations l were encoded as real-valued (x, y) coordinates with (0, 0) being the center of the image x and (-1, -1) being the top left corner of image x.
    \item Glimpse network: The glimpse network $f_g(x;l)$ had two fully connected layers. Let Linear(x) denote a linear transformation of the vector x, i.e. Linear(x) = Wx+b for some weight matrix W and bias vector b, and let Rect(x) = max(x; 0) be the rectifier nonlinearity. The output g of the glimpse network was defined as $g = Rect(Linear(h_g) + Linear(h_l)) where h_g = Rect(Linear(\rho(x; l)))$
    and $h_l = Rect(Linear(l))$. The dimensionality of $h_g$ and $h_l$ are both 128 while dimensionality of g was 256.
    \item Location network: The policy for the locations $l$ was defined by a two-component Gaussian with a fixed variance. The location network outputs the Gaussian sampling around the mean of the location policy at time t and the mean is defined as $f_l(h) = Linear(h)$ where h is the hidden state vector of the core RNN network.
    \item Action network: The output of action network at time t is a 64-dimensional embedding vector, which is defined as $f_a(h) = Linear(h)$ where h is the hidden state vector of the core RNN network.
    \item Core network: A RNN defined as $h_t = f_h(h_{t-1}) = Rect(Linear(h_{t-1}) + Linear(g_t))$.
\end{itemize}

thus making sketching more comparable to traditional search methods in terms of time to issue a query because users can stop drawing whenever they get their desired results\cite{b18}This model assumes an “on-the-fly” setting, in practice, retrieval will be conducted at every stroke drawn.













We will introduce the optimization objective of policy gradient starting from classic theorem in reinforcement learning literature, do some mathematical manipulations, finally deduct its complete form and adjust it to our case. \par
    
    \noindent {\bf The Policy Gradient Theorem:}
    \hitesh{We may need to discuss about our objective function (combined loss) along with the corresponding reward structure and exploration process. Design some function for the reward}
    The derivative of the expected reward is the expectation of the product of the reward and gradient of the log of the policy $\pi_\theta$.
    \begin{equation}
    \nabla \mathrm{E}_{\pi_\theta}[r(\tau)] = \mathrm{E}_{\pi_\theta}[r(\tau)\nabla log\pi_\theta(\tau)]
    \end{equation}
    Now, let us expand the definition of $\pi_\theta(\tau)$.
    \begin{equation}
    \pi_\theta(\tau) = \mathcal{P}(s_0)\prod_{t=1}^{T}\pi_\theta(a_t\vert s_t)p(s_{t+1},r_{t+1}\vert s_t,a_t)
    \end{equation}
    Combining these two equations, to understand this computation, let us break it down - P represents the ergodic distribution of starting in some state $s_0$. From then onwards, we apply the product rule of probability because each new action probability is independent of the previous one (The property of Markov). At each step, we take some action using the policy $\pi_\theta$ and the environment dynamics p decide which new state to transit into. Those are multiplied over T time steps representing the length of the trajectory. Equivalently, taking the log, we have 
    $$
    \begin{aligned}
    log\pi_\theta(\tau) = log\mathcal{P}(s_0)\sum_{t=1}^{T}log\pi_\theta(a_t\vert s_t)\\
    +\sum_{t=1}^{T} log p(s_{t+1},r_{t+1}\vert s_t,a_t)
    \end{aligned}
    $$
    
    $$
    \nabla log\pi_\theta(\tau) = \sum_{t=1}^{T}\nabla log \pi_\theta(a_t\vert s_t)
    $$
    $$
    \longrightarrow \nabla \mathrm{E}_{\pi_\theta}[r(\tau)] = \mathrm{E}_{\pi_\theta}[r(\tau)\sum_{t=1}^{T}\nabla log \pi_\theta(a_t\vert s_t)]
    $$

From this derived formula, we can get the reinforcement learning optimisation object formula in our case:
$$
\begin{aligned}
 \nabla_\theta J = \sum_{t=1}^{T}\mathbb{E}_{p(s_{1:T};\theta)}[\nabla_\theta log\pi (u_t\vert s_{1:t};\theta)R] \\
\approx \frac{1}{M}\sum_{i=1}^{M}\sum_{t=1}^{T}\nabla_\theta log\pi (u_t^i\vert s_{1:t}^i;\theta)R^i
\end{aligned}
$$
    
    In this formula, M represents different episodes, specifically in this project, different sketches to take glimpses on. In every time step t we take one glimpse location $u_t^i$ on the particular sketch, based on the network parameter $\theta$ and the prior knowledge from the previous interactions $s_{1:t}^i$ with the environment, which are encoded by the hidden state vector $h_t$ in our case. For the reward $R^i$, it's the ranking reward mentioned before. It's the same for all the glimpse locations $u_t^i$ because it represents the final retrieval performance based on all glimpse results. Basically, If the ranking reward is high in one episode, then the probability to choose all the glimpse locations $u_t$ of this episode will be trained to increase.
    
    
    And the last, sketch-image hashing\cite{Liu2017,Zhang2018,Shen2018} aims to speed up the computation by converting the final embedding vectors of both branches into binary while not continuous vectors.
    
    
    
    
% 三线表
  \begin{algorithm}[htb]  
  \caption{Training process of Bootstrapped DQN in SBIR setting}  
  \label{alg:DQN}  
  \begin{algorithmic}[1]  
    \Require  
      {$s_0,a_0$,
      $\theta_{policy}^0,\theta_{target}^0,\theta_{locator}^0$}
    \Ensure  
      Optimized $\theta_{policy}^T,\theta_{target}^T,\theta_{locator}^T$
    \For{$t=1;t\leq T;t\leftarrow t+1$}
        
        \State $a_t,r_t,s_{t+1},Q_{policy}(s_t,a_t) = agent(s_t,a_t)$;
        \label{code:agent}  
        \For{Some iterations to find the best action}
         \label{code:for loop1} 
            \State {Fix $\theta_{policy}$, back propagate $Q_{policy}(s_t,a_t)$ to update locator network parameter $\theta_{locator}$}
            \State $a_t,r_t,s_{t+1},Q_{policy}(s_t,a_t) = agent(s_t,a_t)$;
        \EndFor
        \label{code:for loop2} 
        \State Memory add updated ($a_t,r_t,s_t,s_{t+1}$)
        \State $Q^t = Q_{policy}(s_t,a_t)$
        \State {$Q^{t+1} = \mathop{max}\limits_{a_{t+1}}Q_{target}(s_{t+1},a_{t+1})$
        Note: Use \ref{code:for loop1}-\ref{code:for loop2} to find the best action}
        \State Define Loss = $L_1(Q^t-\gamma*Q^{t+1}-r_t)$ to update the $\theta_{policy}$
        
    \EndFor
    
    \State After some episodes, update $\theta_{target}$ using $\theta_{policy}$.\\
    \Return $\theta_{policy}^T,\theta_{target}^T,\theta_{locator}^T$;  
  \end{algorithmic}  
\end{algorithm}  
